Fiducial, total and differential cross-section measurements of $t$-channel single top-quark production in $pp$ collisions at 8 TeV using data collected by the ATLAS detector

Detailed measurements of $t$-channel single top-quark production are presented. They use 20.2 fb$^{-1}$ of data collected by the ATLAS experiment in proton-proton collisions at a centre-of-mass energy of 8 TeV at the LHC. Total, fiducial and differential cross-sections are measured for both top-quark and top-antiquark production. The fiducial cross-section is measured with a precision of 5.8 % (top quark) and 7.8 % (top antiquark), respectively. The total cross-sections are measured to be $\sigma_{\mathrm{tot}}(tq) = 56.7^{+4.3}_{-3.8}\;$pb for top-quark production and $\sigma_{\mathrm{tot}}(\bar{t}q) = 32.9^{+3.0}_{-2.7}\;$pb for top-antiquark production, in agreement with the Standard Model prediction. In addition, the ratio of top-quark to top-antiquark production cross-sections is determined to be $R_t=1.72 \pm 0.09$, with an improved relative precision of 4.9 % since several systematic uncertainties cancel in the ratio. The differential cross-sections as a function of the transverse momentum and rapidity of both the top quark and the top antiquark are measured at both the parton and particle levels. The transverse momentum and rapidity differential cross-sections of the accompanying jet from the $t$-channel scattering are measured at particle level. All measurements are compared to various Monte Carlo predictions as well as to fixed-order QCD calculations where available.

==> auxmat_figs.tex <==
\section{Figures}

This section contains the figures that should be published as auxiliary material.

Distributions of the three most discriminating input variables to the NN without the variable $|\eta(j)|$
after the cut on \NNoutII are shown in \Fig{\ref{fig:CP_NN2a}}.

The statistical correlation matrices are shown in
\Figrange{\ref{fig:correlation_toppt_ptcl}}{\ref{fig:correlation_rap_parton}}.

The normalised unfolded particle-level cross-sections for top quarks and top antiquarks as a function of
\pTthat are shown in \Fig{\ref{fig:xsectN:pTt:particle}},
while the cross-sections as a function of \absythat are shown in \Fig{\ref{fig:xsectN:yt:particle}}.
The normalised unfolded cross-sections for the untagged jet as a function of the same variables 
are shown in \Figs{\ref{fig:xsectN:pTjt:particle}}{\ref{fig:xsectN:yjt:particle}}.
The normalised unfolded parton-level cross-sections as a function of \pTt and \yt are shown in \Figs{\ref{fig:xsectN:pTt:parton}}{\ref{fig:xsectN:yt:parton}}.

%-------------------------------------------------------------------------------
% NN variable distributions
%-------------------------------------------------------------------------------

\begin{figure} [htbp]
  \centering
  \subfloat[][]{
    \includegraphics[trim={0 0 0 30pt}, clip, width=0.42\textwidth]{BillFitCP_plus_2ndNN/mj1j2_Stacked_NormBillFit}
  }
  \subfloat[][]{
    \includegraphics[trim={0 0 0 30pt}, clip, width=0.42\textwidth]{BillFitCP_minus_2ndNN/mj1j2_Stacked_NormBillFit}
  }\\
  \subfloat[][]{
    \includegraphics[trim={0 0 0 30pt}, clip, width=0.42\textwidth]{BillFitCP_plus_2ndNN/mlnub_Stacked_NormBillFit}
  }
  \subfloat[][]{
    \includegraphics[trim={0 0 0 30pt}, clip, width=0.42\textwidth]{BillFitCP_minus_2ndNN/mlnub_Stacked_NormBillFit}
  }\\
  \subfloat[][]{
    \includegraphics[trim={0 0 0 30pt}, clip, width=0.42\textwidth]{BillFitCP_plus_2ndNN/mtw_Stacked_NormBillFit}
  }
  \subfloat[][]{
    \includegraphics[trim={0 0 0 30pt}, clip, width=0.42\textwidth]{BillFitCP_minus_2ndNN/mtw_Stacked_NormBillFit}
  }
  \caption{Observed distributions of the first three input variables to the neural network without $|\eta(j)|$
    in the signal region (SR), after a cut of $\NNoutII > 0.8$ on the network output.
    The distributions are compared to the model obtained from simulated events.
    The simulated distributions are normalised to
    the event rates obtained by the fit to the discriminants.
    The definitions of the variables can be found in \Tab{\ref{tab:NNinputVars}}.
    \postfitCaptionUncSentence 
    Events beyond the $x$-axis range in (a) and (b) are included in the last bin.
    The lower panels show the ratio between the observed and the expected number of events in each bin to
    illustrate the goodness-of-fit.
  }
  \label{fig:CP_NN2a}
\end{figure}

%-------------------------------------------------------------------------------
% Correlation matrices
%-------------------------------------------------------------------------------

\begin{figure}[htbp]
	\centering
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/topPt_plus/topPtRB1_asym_recocorrelationmatrix_allsys_2D}}\quad
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/topPt_minus/topPtRB5_asym_recocorrelationmatrix_allsys_2D}} \\
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/topPt_plus/topPtRB1_asym_recocorrelationmatrix_allsys_NormXS_2D}}\quad
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/topPt_minus/topPtRB5_asym_recocorrelationmatrix_allsys_NormXS_2D}}	
  \caption{Statistical correlation matrix for the absolute differential cross-sections as a function of \pTthat for
    (a) \tq and (b) \tbarq events as well as for the normalised differential cross-sections
    for (c) \tq and (d) \tbarq events.  
    It includes the statistical uncertainty due to the number of data events and MC statistics.
  }
  \label{fig:correlation_toppt_ptcl}
\end{figure}

\begin{figure}[htbp]
	\centering
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/topRap_plus/topAbsRapRB16_asym_recocorrelationmatrix_allsys_2D}}\quad
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/topRap_minus/topAbsRapRB16_asym_recocorrelationmatrix_allsys_2D}} \\
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/topRap_plus/topAbsRapRB16_asym_recocorrelationmatrix_allsys_NormXS_2D}}\quad
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/topRap_minus/topAbsRapRB16_asym_recocorrelationmatrix_allsys_NormXS_2D}}	
  \caption{Statistical correlation matrix for the absolute differential cross-sections as a function of \absythat for
    (a) \tq and (b) \tbarq events as well as for the normalised differential cross-sections
    for (c) \tq and (d) \tbarq events.
    It includes the statistical uncertainty due to the number of data events and MC statistics.
  }
  \label{fig:correlation_toprap_ptcl}
\end{figure}

\begin{figure}[htbp]
	\centering
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/lightjetPt_plus/lightPtRB1_asym_recocorrelationmatrix_allsys_2D}}\quad
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/lightjetPt_minus/lightPtRB1_asym_recocorrelationmatrix_allsys_2D}} \\
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/lightjetPt_plus/lightPtRB1_asym_recocorrelationmatrix_allsys_NormXS_2D}}\quad
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/lightjetPt_minus/lightPtRB1_asym_recocorrelationmatrix_allsys_NormXS_2D}}	
  \caption{Statistical correlation matrix for the absolute differential cross-sections as a function of \pTjhat for
    (a) \tq and (b) \tbarq events as well as for the normalised differential cross-sections
    for (c) \tq and (d) \tbarq events.
    It includes the statistical uncertainty due to the number of data events and MC statistics.
  }
  \label{fig:correlation_lightpt_ptcl}
\end{figure}

\begin{figure}[htbp]
	\centering
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/lightjetRap_plus/lightAbsRapRB8_asym_recocorrelationmatrix_allsys_2D}}\quad
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/lightjetRap_minus/lightAbsRapRB8_asym_recocorrelationmatrix_allsys_2D}} \\
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/lightjetRap_plus/lightAbsRapRB8_asym_recocorrelationmatrix_allsys_NormXS_2D}}\quad
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/lightjetRap_minus/lightAbsRapRB8_asym_recocorrelationmatrix_allsys_NormXS_2D}}	
  \caption{Statistical correlation matrix for the absolute differential cross-sections as a function of \absyjhat for
    (a) \tq and (b) \tbarq events as well as for the normalised differential cross-sections
    for (c) \tq and (d) \tbarq events.
    It includes the statistical uncertainty due to the number of data events and MC statistics.
  }
  \label{fig:correlation_lightrap_ptcl}
\end{figure}


\begin{figure}[htbp]
	\centering
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{PtBinning/topPtRB2_plus/topPtRB2_asym_recocorrelationmatrix_allsys_2D}}\quad
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{PtBinning/topPtRB6_minus/topPtRB6_asym_recocorrelationmatrix_allsys_2D}} \\
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{PtBinning/topPtRB2_plus/topPtRB2_asym_recocorrelationmatrix_allsys_NormXS_2D}}\quad
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{PtBinning/topPtRB6_minus/topPtRB6_asym_recocorrelationmatrix_allsys_NormXS_2D}}	
  \caption{Statistical correlation matrix for the absolute differential cross-sections as a function of \pTt for
    (a) \tq and (b) \tbarq events as well as for the normalised differential cross-sections
    for (c) \tq and (d) \tbarq events.
    It includes the statistical uncertainty due to the number of data events and MC statistics.
  }
  \label{fig:correlation_pt_parton}
\end{figure}

\begin{figure}[htbp]
	\centering
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{RapBinning/RapRB5_plus/topAbsRapRB5_asym_recocorrelationmatrix_allsys_2D}}\quad
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{RapBinning/RapRB5_minus/topAbsRapRB5_asym_recocorrelationmatrix_allsys_2D}} \\
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{RapBinning/RapRB5_plus/topAbsRapRB5_asym_recocorrelationmatrix_allsys_NormXS_2D}}\quad
	\subfloat[][]{\includegraphics[width=0.46\textwidth]{RapBinning/RapRB5_minus/topAbsRapRB5_asym_recocorrelationmatrix_allsys_NormXS_2D}}	
  \caption{Statistical correlation matrix for the absolute differential cross-sections as a function of \absyt for
    (a) \tq and (b) \tbarq events as well as for the normalised differential cross-sections 
    for (c) \tq and (d) \tbarq events.
    It includes the statistical uncertainty due to the number of data events and MC statistics.
  }
  \label{fig:correlation_rap_parton}
\end{figure}

%-------------------------------------------------------------------------------
% Normalised cross-sections
%-------------------------------------------------------------------------------

\begin{figure}[htbp]
  \centering
  %\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/topPt_plus/toppt_sub_logy}}\quad
  %\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/topPt_minus/antitoppt_sub_logy}}\\
  \subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/topPt_plus/toppt_sub_norm_logy}}\quad
  \subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/topPt_minus/antitoppt_sub_norm_logy}}
  \caption{Normalised unfolded differential cross-sections as a function of \pTthat for
    (a) top quarks and (b) top antiquarks.
    \DiffXsectFigCaption
  }
  \label{fig:xsectN:pTt:particle}
\end{figure}

\begin{figure}[htbp]
  \centering
  %\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/topRap_plus/toprapidity_sub}}\quad
  %\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/topRap_minus/antitoprapidity_sub}}\\
  \subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/topRap_plus/toprapidity_sub_norm}}\quad
  \subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/topRap_minus/antitoprapidity_sub_norm}}
  \caption{Normalised unfolded differential cross-sections as a function of \absythat for
    (a) top quarks and (b) top antiquarks.
    \DiffXsectFigCaption
  }
  \label{fig:xsectN:yt:particle}
\end{figure}

\begin{figure}[htbp]
  \centering
  %\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/lightjetPt_plus/topptlight_sub_logy}}\quad
  %\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/lightjetPt_minus/antitopptlight_sub_logy}}\\
  \subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/lightjetPt_plus/topptlight_sub_norm_logy}}\quad
  \subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/lightjetPt_minus/antitopptlight_sub_norm_logy}}
  \caption{Normalised unfolded differential cross-sections as a function of \pTjhat for
    (a) top quarks (b) top antiquarks.
    \DiffXsectFigCaption
  }
  \label{fig:xsectN:pTjt:particle}
\end{figure}

\begin{figure}[htbp]
  \centering
  %\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/lightjetRap_plus/toprapiditylight_sub}}\quad
  %\subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/lightjetRap_minus/antitoprapiditylight_sub}}\\
  \subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/lightjetRap_plus/toprapiditylight_sub_norm}}\quad
  \subfloat[][]{\includegraphics[width=0.46\textwidth]{unfoldtoFid/lightjetRap_minus/antitoprapiditylight_sub_norm}}
  \caption{Normalised unfolded differential cross-sections as a function of \absyjhat for
    (a) top quarks and (b) top antiquarks.
    \DiffXsectFigCaption
  }
  \label{fig:xsectN:yjt:particle}
\end{figure}

\begin{figure}[htbp]
  \centering
  %\subfloat[][]{\includegraphics[width=0.46\textwidth]{PtBinning/topPtRB2_plus/toppt_sub_logyKidonakis}}\quad
  %\subfloat[][]{\includegraphics[width=0.46\textwidth]{PtBinning/topPtRB6_minus/antitoppt_sub_logyKidonakis}}\\
  \subfloat[][]{\includegraphics[width=0.46\textwidth]{PtBinning/topPtRB2_plus/toppt_sub_norm_logyKidonakis}}\quad
  \subfloat[][]{\includegraphics[width=0.46\textwidth]{PtBinning/topPtRB6_minus/antitoppt_sub_norm_logyKidonakis}}
  \caption{Normalised unfolded differential cross-sections as a function of \pTt for
    (a) top quarks and (b) top antiquarks.
    The unfolded distributions are compared to QCD N(N)LO calculations and various MC predictions. 
    \DiffXsectpTFigCaption
  }
  \label{fig:xsectN:pTt:parton}
\end{figure}

\begin{figure}[htbp]
  \centering
  %\subfloat[][]{\includegraphics[width=0.46\textwidth]{RapBinning/RapRB5_plus/toprapidity_sub}}\quad  
  %\subfloat[][]{\includegraphics[width=0.46\textwidth]{RapBinning/RapRB5_minus/antitoprapidity_sub}}\\
  \subfloat[][]{\includegraphics[width=0.46\textwidth]{RapBinning/RapRB5_plus/toprapidity_sub_norm}}\quad
  \subfloat[][]{\includegraphics[width=0.46\textwidth]{RapBinning/RapRB5_minus/antitoprapidity_sub_norm}}
  \caption{Normalised unfolded differential cross-sections as a function of \absyt for
    (a) top quarks and (b) top antiquarks.
    The unfolded distributions are compared to a QCD NLO calculation and various MC predictions. 
    \DiffXsectEtaFigCaption
  }
  \label{fig:xsectN:yt:parton}
\end{figure}



==> auxmat_tables.tex <==
\section{Tables}

This section contains the tables that should be published as auxiliary material.

\Tabs{\ref{tab:fid_acc_top}}{\ref{tab:fid_acc_antitop}} contain the fiducial
acceptances $A_\text{fid}$, obtained for several MC event generators, separated
into top quark $t$-channel single top-quark and top-antiquark. The corresponding
scale and PDF uncertainties for the individual samples are shown.

\begin{table}[htbp]
  \centering
  \sisetup{retain-explicit-plus}
   %\setlength{\tabcolsep}{1mm}
   \begin{tabular}{llc
     S
     S[table-format=-1.1]@{\,/\,}S[table-format=-1.1]
     S}
   \toprule
   ME Generator & Shower MC &  Method & {$A_\text{fid}(\tq)$} & \multicolumn{2}{c}{Scale unc.} & {PDF unc.} \\
   & & & {[\%]} & \multicolumn{2}{c}{[\%]} & {[\%]}\\
   \toprule    
   \POWHEGBOX  & \PYTHIAV{6}  & 4FS(NLO)    & 17.3  & +0.5 & -0.2 &  \pm 0.10$^{\text{(a)}}$\\
   \POWHEGBOX  & \PYTHIAV{8}  & 4FS(NLO)    & 17.2  & +0.5 & -0.2$^{\text{(b)}}$ &  \pm 0.10$^{\text{(a)}}$\\
   \POWHEGBOX  & \HERWIG      & 4FS(NLO)    & 17.1  & +0.5 & -0.2$^{\text{(b)}}$ &  \pm 0.10$^{\text{(a)}}$\\
   \POWHEGBOX  & \HERWIGV{7}  & 4FS(NLO)    & 15.7  & +0.1 & -0.1 &  \pm 0.10$^{\text{(a)}}$\\
   \MGMCatNLO  & \HERWIG      & 4FS(NLO)    & 16.9  & +0.5 & -0.2$^{\text{(b)}}$ & \pm 0.10$^{\text{(a)}}$\\
   \MGMCatNLO  & \HERWIGV{7}  & 4FS(NLO)    & 18.4  & +0.5 & -0.2$^{\text{(b)}}$ & \pm 0.10$^{\text{(a)}}$ \\
   \midrule
   \POWHEGBOX  & \PYTHIAV{6}  & 5FS(NLO)    & 17.2  & +0.9 & -0.2 &  \pm 0.10$^{\text{(a)}}$\\
   \POWHEGBOX  & \PYTHIAV{8}  & 5FS(NLO)    & 17.3  & +0.5 & -0.3 &  \pm 0.10$^{\text{(a)}}$ \\
   \MGMCatNLO  & \HERWIGV{7}  & 5FS(NLO)    & 16.2  & +0.3 & -0.3 &  \pm 0.10$^{\text{(a)}}$ \\
   \bottomrule
   \end{tabular}
  \caption{Fiducial acceptance $A_\text{fid}$ for different $t$-channel single top-quark MC samples.
  $^{\text{(a)}}$ Calculation taken from \ACERMC + \PYTHIAV{6}. $^{\text{(b)}}$ Calculation taken from \POWHEGBOX + \PYTHIAV{6}.     
   \label{tab:fid_acc_top}}
\end{table}


\begin{table}[htbp]
  \centering
   \setlength{\tabcolsep}{1mm}
   \begin{tabular}{llc
     S
     S[table-format=-1.1]@{\,/\,}S[table-format=-1.1]
     S}
   \toprule
   ME Generator & Shower MC &  Method & {$A_\text{fid}(\tbarq)$} & \multicolumn{2}{c}{Scale unc.} & {PDF unc.} \\
   & & & {[\%]} & \multicolumn{2}{c}{[\%]} & {[\%]}\\
   \toprule    
   \POWHEGBOX & \PYTHIAV{6}  & 4FS(NLO)    & 17.5 & +0.2 & -0.4 & \pm 0.16$^{\text{(a)}}$ \\
   \POWHEGBOX & \PYTHIAV{8}  & 4FS(NLO)    & 17.5 & +0.2 & -0.4$^{\text{(b)}}$ &  \pm 0.16$^{\text{(a)}}$ \\
   \POWHEGBOX & \HERWIG      & 4FS(NLO)    & 17.4 & +0.2 & -0.4$^{\text{(b)}}$ &  \pm 0.16$^{\text{(a)}}$\\
   \POWHEGBOX & \HERWIGV{7}  & 4FS(NLO)    & 16.7 & +0.1 & -0.1 &  \pm 0.16$^{\text{(a)}}$\\
   \MGMCatNLO & \HERWIG      & 4FS(NLO)    & 17.1 & +0.2 & -0.4$^{\text{(b)}}$ & \pm 0.16$^{\text{(a)}}$   \\
   \MGMCatNLO & \HERWIGV{7}  & 4FS(NLO)    & 18.3 & +0.2 & -0.4$^{\text{(b)}}$ & \pm 0.16$^{\text{(a)}}$   \\
   \midrule
   \POWHEGBOX  & \PYTHIAV{6} & 5FS(NLO)    & 18.0 & +0.1 & -0.2 & \pm 0.16$^{\text{(a)}}$  \\
   \POWHEGBOX  & \PYTHIAV{8} & 5FS(NLO)    & 17.8 & +0.2 & -0.3 & \pm 0.16$^{\text{(a)}}$  \\
   \MGMCatNLO  & \HERWIGV{7} & 5FS(NLO)    & 17.1 & +0.4 & -0.3 & \pm 0.16$^{\text{(a)}}$  \\
   \bottomrule
   \end{tabular}
  \caption{Fiducial acceptance $A_\text{fid}$ for different $t$-channel single top-antiquark MC samples.
    $^{\text{(a)}}$ Calculation taken from \ACERMC + \PYTHIAV{6}. $^{\text{(b)}}$ Calculation taken from \POWHEGBOX + \PYTHIAV{6}.
   \label{tab:fid_acc_antitop}}
\end{table}

==> systopPt_minus_XS_summary.tex <==
Source of uncertainty      & \multicolumn{2}{c}{Bin 1}      & \multicolumn{2}{c}{Bin 2}      & \multicolumn{2}{c}{Bin 3}      & \multicolumn{2}{c}{Bin 4}         \\
& \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}     \\
\midrule
\endhead
  Data statistics & \symerr{5.0} & \symerr{6.7} & \symerr{12} & \symerr{20} \\
  Monte Carlo statistics & \symerr{0.4} & \symerr{0.5} & \symerr{1.1} & \symerr{1.7} \\
\midrule
  Unfolding & \asymerr{+3.7}{-3.7} & \asymerr{+4.5}{-4.5} & \asymerr{+3.5}{-3.5} & \asymerr{+6.7}{-6.7} \\
  Background normalisation & \asymerr{+0.3}{-0.3} & \asymerr{+1.1}{-1.1} & \asymerr{+0.6}{-0.6} & \asymerr{+4.2}{-4.2} \\
  Background modelling & \asymerr{+1.3}{-1.3} & \asymerr{+0.8}{-0.8} & \asymerr{+3.3}{-3.3} & \asymerr{+1.6}{-1.6} \\
  Lepton reconstruction & \asymerr{+0.3}{-0.1} & \asymerr{+0.1}{-0.4} & \asymerr{+0.4}{-0.5} & \asymerr{+0.6}{-0.3} \\
  Jet reconstruction & \asymerr{+2.7}{-2.7} & \asymerr{+3.2}{-3.2} & \asymerr{+0.8}{-0.8} & \asymerr{+1.8}{-1.8} \\
  Jet energy scale & \asymerr{+1.6}{-0.6} & \asymerr{+0.2}{-1.7} & \asymerr{+2.4}{-1.5} & \asymerr{+2.5}{-2.5} \\
  Flavour tagging & \asymerr{+0.3}{-0.3} & \asymerr{+0.2}{-0.2} & \asymerr{+0.5}{-0.5} & \asymerr{+0.8}{-0.9} \\
  \MET modelling & \asymerr{+0.5}{-0.4} & \asymerr{+0.0}{-0.2} & \asymerr{+1.1}{-0.7} & \asymerr{+0.8}{-0.9} \\
  PDF & \asymerr{+2.3}{-2.3} & \asymerr{+1.8}{-1.9} & \asymerr{+3.5}{-3.4} & \asymerr{+2.3}{-2.3} \\
  \tq (\tbarq) NLO matching & \asymerr{+5.3}{-5.3} & \asymerr{+2.2}{-2.2} & \asymerr{+17}{-17} & \asymerr{+11}{-11} \\
  \tq (\tbarq) parton shower & \asymerr{+1.0}{-1.0} & \asymerr{+0.8}{-0.8} & \asymerr{+1.8}{-1.8} & \asymerr{+0.8}{-0.8} \\
  \tq (\tbarq) scale variations & \asymerr{+1.3}{-1.9} & \asymerr{+1.8}{-1.0} & \asymerr{+0.2}{-0.0} & \asymerr{+2.7}{-3.7} \\
  \ttbar NLO matching & \asymerr{+0.8}{-0.8} & \asymerr{+1.5}{-1.5} & \asymerr{+1.8}{-1.8} & \asymerr{+17}{-17} \\
  \ttbar parton shower & \asymerr{+0.6}{-0.6} & \asymerr{+1.1}{-1.1} & \asymerr{+4.5}{-4.5} & \asymerr{+15}{-15} \\
  \ttbar scale variations & \asymerr{+0.8}{-0.0} & \asymerr{+0.0}{-1.8} & \asymerr{+0.0}{-3.4} & \asymerr{+17}{-0} \\
\midrule
  Total systematic & \asymerr{+8.0}{-7.9} & \asymerr{+6.9}{-7.2} & \asymerr{+19}{-19} & \asymerr{+31}{-27} \\
  Total (stat.\ + syst.) & \asymerr{+9.4}{-9.4} & \asymerr{+10}{-10} & \asymerr{+22}{-22} & \asymerr{+37}{-33} \\


==> systopPt_minus_summary.tex <==
Source of uncertainty      & \multicolumn{2}{c}{Bin 1}      & \multicolumn{2}{c}{Bin 2}      & \multicolumn{2}{c}{Bin 3}      & \multicolumn{2}{c}{Bin 4}         \\
& \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}     \\
\midrule
\endhead
  Data statistics & \symerr{7.0} & \symerr{5.8} & \symerr{12} & \symerr{20} \\
  Monte Carlo statistics & \symerr{0.7} & \symerr{0.6} & \symerr{1.1} & \symerr{1.7} \\
\midrule
  Unfolding & \asymerr{+3.9}{-3.9} & \asymerr{+4.3}{-4.3} & \asymerr{+3.7}{-3.7} & \asymerr{+6.5}{-6.5} \\
  Background normalisation & \asymerr{+5.8}{-5.8} & \asymerr{+4.5}{-4.5} & \asymerr{+6.1}{-6.1} & \asymerr{+10}{-10} \\
  Background modelling & \asymerr{+1.4}{-1.4} & \asymerr{+0.6}{-0.6} & \asymerr{+3.2}{-3.2} & \asymerr{+1.8}{-1.8} \\
  Lepton reconstruction & \asymerr{+1.9}{-1.9} & \asymerr{+1.9}{-1.9} & \asymerr{+2.0}{-2.0} & \asymerr{+1.9}{-1.9} \\
  Jet reconstruction & \asymerr{+2.3}{-2.3} & \asymerr{+3.5}{-3.5} & \asymerr{+1.1}{-1.1} & \asymerr{+2.1}{-2.1} \\
  Jet energy scale & \asymerr{+2.9}{-1.1} & \asymerr{+2.0}{-3.1} & \asymerr{+3.9}{-2.4} & \asymerr{+3.4}{-2.8} \\
  Flavour tagging & \asymerr{+1.2}{-1.2} & \asymerr{+1.1}{-1.1} & \asymerr{+1.3}{-1.3} & \asymerr{+1.4}{-1.4} \\
  \MET modelling & \asymerr{+0.9}{-0.6} & \asymerr{+0.1}{-0.3} & \asymerr{+1.0}{-0.3} & \asymerr{+0.6}{-0.5} \\
  $b/\bbar$ efficiency & \symerr{0.9} & \symerr{0.9} & \symerr{0.9} & \symerr{0.9} \\
  PDF & \asymerr{+2.9}{-2.9} & \asymerr{+1.2}{-1.3} & \asymerr{+2.8}{-2.8} & \asymerr{+2.7}{-2.7} \\
  \tq (\tbarq) NLO matching & \asymerr{+6.7}{-6.7} & \asymerr{+0.8}{-0.8} & \asymerr{+16}{-16} & \asymerr{+12}{-12} \\
  \tq (\tbarq) parton shower & \asymerr{+1.4}{-1.4} & \asymerr{+0.4}{-0.4} & \asymerr{+1.5}{-1.5} & \asymerr{+1.2}{-1.2} \\
  \tq (\tbarq) scale variations & \asymerr{+1.6}{-2.3} & \asymerr{+1.4}{-0.7} & \asymerr{+0.5}{-0.4} & \asymerr{+2.2}{-3.4} \\
  \ttbar NLO matching & \asymerr{+0.7}{-0.7} & \asymerr{+1.4}{-1.4} & \asymerr{+1.9}{-1.9} & \asymerr{+17}{-17} \\
  \ttbar parton shower & \asymerr{+1.0}{-1.0} & \asymerr{+0.8}{-0.8} & \asymerr{+4.2}{-4.2} & \asymerr{+15}{-15} \\
  \ttbar scale variations & \asymerr{+1.2}{-0.0} & \asymerr{+0.0}{-1.5} & \asymerr{+0.0}{-3.1} & \asymerr{+17}{-0} \\
  Luminosity & \symerr{1.9} & \symerr{1.9} & \symerr{1.9} & \symerr{1.9} \\
\midrule
  Total systematic & \asymerr{+12}{-11} & \asymerr{+8.5}{-8.9} & \asymerr{+19}{-19} & \asymerr{+34}{-29} \\
  Total (stat.\ + syst.) & \asymerr{+14}{-13} & \asymerr{+10}{-11} & \asymerr{+22}{-22} & \asymerr{+39}{-35} \\


==> systopPt_plus_XS_summary.tex <==
Source of uncertainty      & \multicolumn{2}{c}{Bin 1}      & \multicolumn{2}{c}{Bin 2}      & \multicolumn{2}{c}{Bin 3}      & \multicolumn{2}{c}{Bin 4} & \multicolumn{2}{c}{Bin 5}        \\
& \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}  & \multicolumn{2}{c}{[\%]}      \\
\midrule
\endhead
  Data statistics & \symerr{3.9} & \symerr{4.3} & \symerr{6.7} & \symerr{13} & \symerr{19} \\
  Monte Carlo statistics & \symerr{0.5} & \symerr{0.5} & \symerr{0.9} & \symerr{1.6} & \symerr{2.4} \\
\midrule
  Unfolding & \asymerr{+1.6}{-1.6} & \asymerr{+1.3}{-1.3} & \asymerr{+1.9}{-1.9} & \asymerr{+0.5}{-0.5} & \asymerr{+1.3}{-1.3} \\
  Background normalisation & \asymerr{+1.1}{-1.1} & \asymerr{+1.0}{-1.0} & \asymerr{+0.5}{-0.5} & \asymerr{+0.9}{-0.9} & \asymerr{+0.5}{-0.5} \\
  Background modelling & \asymerr{+0.7}{-0.7} & \asymerr{+0.5}{-0.5} & \asymerr{+1.1}{-1.1} & \asymerr{+1.2}{-1.2} & \asymerr{+0.3}{-0.3} \\
  Lepton reconstruction & \asymerr{+0.0}{-0.1} & \asymerr{+0.1}{-0.2} & \asymerr{+0.6}{-0.2} & \asymerr{+0.6}{-0.2} & \asymerr{+0.3}{-0.8} \\
  Jet reconstruction & \asymerr{+0.1}{-0.1} & \asymerr{+0.3}{-0.3} & \asymerr{+0.4}{-0.4} & \asymerr{+0.3}{-0.3} & \asymerr{+1.7}{-1.7} \\
  Jet energy scale & \asymerr{+1.7}{-1.2} & \asymerr{+1.0}{-1.3} & \asymerr{+1.4}{-2.3} & \asymerr{+4.9}{-2.0} & \asymerr{+1.1}{-5.7} \\
  Flavour tagging & \asymerr{+0.3}{-0.3} & \asymerr{+0.1}{-0.1} & \asymerr{+0.5}{-0.5} & \asymerr{+0.7}{-0.7} & \asymerr{+1.1}{-1.1} \\
  \MET modelling & \asymerr{+0.4}{-0.1} & \asymerr{+0.1}{-0.1} & \asymerr{+0.6}{-1.2} & \asymerr{+1.5}{-0.0} & \asymerr{+0.0}{-1.8} \\
  PDF & \asymerr{+0.6}{-0.7} & \asymerr{+0.4}{-0.3} & \asymerr{+0.6}{-0.6} & \asymerr{+1.7}{-1.7} & \asymerr{+1.2}{-1.2} \\
  \tq (\tbarq) NLO matching & \asymerr{+1.6}{-1.6} & \asymerr{+4.2}{-4.2} & \asymerr{+8.4}{-8.4} & \asymerr{+4.3}{-4.3} & \asymerr{+3.3}{-3.3} \\
  \tq (\tbarq) parton shower & \asymerr{+0.7}{-0.7} & \asymerr{+1.8}{-1.8} & \asymerr{+2.9}{-2.9} & \asymerr{+0.6}{-0.6} & \asymerr{+1.9}{-1.9} \\
  \tq (\tbarq) scale variations & \asymerr{+1.6}{-3.9} & \asymerr{+3.7}{-0.0} & \asymerr{+1.5}{-4.2} & \asymerr{+0.9}{-4.0} & \asymerr{+3.5}{-0.8} \\
  \ttbar NLO matching & \asymerr{+0.4}{-0.4} & \asymerr{+0.6}{-0.6} & \asymerr{+2.3}{-2.3} & \asymerr{+3.0}{-3.0} & \asymerr{+6.6}{-6.6} \\
  \ttbar parton shower & \asymerr{+0.0}{-0.0} & \asymerr{+0.5}{-0.5} & \asymerr{+0.1}{-0.1} & \asymerr{+1.6}{-1.6} & \asymerr{+4.3}{-4.3} \\
  \ttbar scale variations & \asymerr{+0.5}{-0.0} & \asymerr{+0.0}{-1.5} & \asymerr{+1.7}{-0.0} & \asymerr{+3.4}{-0.0} & \asymerr{+0.0}{-3.6} \\
\midrule
  Total systematic & \asymerr{+3.7}{-5.0} & \asymerr{+6.3}{-5.4} & \asymerr{+10}{-11} & \asymerr{+8.8}{-7.7} & \asymerr{+10}{-12} \\
  Total (stat.\ + syst.) & \asymerr{+5.4}{-6.4} & \asymerr{+7.6}{-6.9} & \asymerr{+12}{-13} & \asymerr{+16}{-15} & \asymerr{+21}{-22} \\


==> systopPt_plus_summary.tex <==
Source of uncertainty      & \multicolumn{2}{c}{Bin 1}      & \multicolumn{2}{c}{Bin 2}      & \multicolumn{2}{c}{Bin 3}      & \multicolumn{2}{c}{Bin 4} & \multicolumn{2}{c}{Bin 5}        \\
& \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}  & \multicolumn{2}{c}{[\%]}      \\
\midrule
\endhead
  Data statistics & \symerr{5.4} & \symerr{3.8} & \symerr{6.8} & \symerr{13} & \symerr{19} \\
  Monte Carlo statistics & \symerr{0.7} & \symerr{0.5} & \symerr{0.9} & \symerr{1.6} & \symerr{2.4} \\
\midrule
  Unfolding & \asymerr{+2.0}{-2.0} & \asymerr{+0.9}{-0.9} & \asymerr{+1.5}{-1.5} & \asymerr{+0.9}{-0.9} & \asymerr{+1.7}{-1.7} \\
  Background normalisation & \asymerr{+4.6}{-4.6} & \asymerr{+2.6}{-2.6} & \asymerr{+3.0}{-3.0} & \asymerr{+2.7}{-2.7} & \asymerr{+4.0}{-4.0} \\
  Background modelling & \asymerr{+0.8}{-0.8} & \asymerr{+0.5}{-0.5} & \asymerr{+1.0}{-1.0} & \asymerr{+1.3}{-1.3} & \asymerr{+0.4}{-0.4} \\
  Lepton reconstruction & \asymerr{+1.9}{-1.9} & \asymerr{+1.9}{-1.9} & \asymerr{+2.0}{-1.9} & \asymerr{+1.9}{-1.9} & \asymerr{+2.0}{-2.1} \\
  Jet reconstruction & \asymerr{+1.1}{-1.1} & \asymerr{+1.5}{-1.5} & \asymerr{+0.8}{-0.8} & \asymerr{+0.9}{-0.9} & \asymerr{+2.9}{-2.9} \\
  Jet energy scale & \asymerr{+2.0}{-1.7} & \asymerr{+2.2}{-2.6} & \asymerr{+1.9}{-2.2} & \asymerr{+6.0}{-2.4} & \asymerr{+1.0}{-5.6} \\
  Flavour tagging & \asymerr{+1.2}{-1.2} & \asymerr{+1.2}{-1.2} & \asymerr{+1.2}{-1.2} & \asymerr{+1.4}{-1.4} & \asymerr{+1.4}{-1.4} \\
  \MET modelling & \asymerr{+0.6}{-0.3} & \asymerr{+0.2}{-0.2} & \asymerr{+0.6}{-1.0} & \asymerr{+1.3}{-0.0} & \asymerr{+0.0}{-1.9} \\
  $b/\bbar$ efficiency & \symerr{0.9} & \symerr{0.9} & \symerr{0.9} & \symerr{0.9} & \symerr{0.9} \\
  PDF & \asymerr{+0.8}{-0.9} & \asymerr{+0.2}{-0.1} & \asymerr{+0.4}{-0.4} & \asymerr{+1.5}{-1.5} & \asymerr{+1.1}{-1.1} \\
  \tq (\tbarq) NLO matching & \asymerr{+2.2}{-2.2} & \asymerr{+3.7}{-3.7} & \asymerr{+8.9}{-8.9} & \asymerr{+3.8}{-3.8} & \asymerr{+2.8}{-2.8} \\
  \tq (\tbarq) parton shower & \asymerr{+0.9}{-0.9} & \asymerr{+1.6}{-1.6} & \asymerr{+3.1}{-3.1} & \asymerr{+0.8}{-0.8} & \asymerr{+1.7}{-1.7} \\
  \tq (\tbarq) scale variations & \asymerr{+2.0}{-4.9} & \asymerr{+2.6}{-0.0} & \asymerr{+0.4}{-3.9} & \asymerr{+0.0}{-3.6} & \asymerr{+3.8}{-1.9} \\
  \ttbar NLO matching & \asymerr{+0.4}{-0.4} & \asymerr{+0.5}{-0.5} & \asymerr{+2.3}{-2.3} & \asymerr{+3.0}{-3.0} & \asymerr{+6.6}{-6.6} \\
  \ttbar parton shower & \asymerr{+0.1}{-0.1} & \asymerr{+0.4}{-0.4} & \asymerr{+0.1}{-0.1} & \asymerr{+1.6}{-1.6} & \asymerr{+4.3}{-4.3} \\
  \ttbar scale variations & \asymerr{+0.7}{-0.0} & \asymerr{+0.0}{-1.4} & \asymerr{+1.8}{-0.0} & \asymerr{+3.5}{-0.0} & \asymerr{+0.0}{-3.4} \\
  Luminosity & \symerr{1.9} & \symerr{1.9} & \symerr{1.9} & \symerr{1.9} & \symerr{1.9} \\
\midrule
  Total systematic & \asymerr{+7.2}{-8.4} & \asymerr{+6.9}{-6.7} & \asymerr{+11}{-12} & \asymerr{+10}{-8} & \asymerr{+12}{-13} \\
  Total (stat.\ + syst.) & \asymerr{+9.0}{-10.0} & \asymerr{+7.9}{-7.7} & \asymerr{+13}{-14} & \asymerr{+16}{-15} & \asymerr{+22}{-23} \\


==> systopY_minus_XS_summary.tex <==
Source of uncertainty      & \multicolumn{2}{c}{Bin 1}      & \multicolumn{2}{c}{Bin 2}      & \multicolumn{2}{c}{Bin 3}      & \multicolumn{2}{c}{Bin 4}        \\
& \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}        \\
\midrule
\endhead
  Data statistics & \symerr{7.7} & \symerr{8.5} & \symerr{6.9} & \symerr{10} \\
  Monte Carlo statistics & \symerr{0.8} & \symerr{0.7} & \symerr{0.6} & \symerr{0.9} \\
\midrule
  Unfolding & \asymerr{+0.5}{-0.5} & \asymerr{+0.1}{-0.1} & \asymerr{+3.1}{-3.1} & \asymerr{+4.7}{-4.7} \\
  Background normalisation & \asymerr{+1.7}{-1.7} & \asymerr{+0.5}{-0.5} & \asymerr{+0.4}{-0.4} & \asymerr{+3.1}{-3.1} \\
  Background modelling & \asymerr{+0.8}{-0.8} & \asymerr{+0.4}{-0.4} & \asymerr{+2.0}{-2.0} & \asymerr{+3.4}{-3.4} \\
  Lepton reconstruction & \asymerr{+0.3}{-0.2} & \asymerr{+0.6}{-0.3} & \asymerr{+0.2}{-0.4} & \asymerr{+0.4}{-0.4} \\
  Jet reconstruction & \asymerr{+0.3}{-0.3} & \asymerr{+0.1}{-0.1} & \asymerr{+0.7}{-0.7} & \asymerr{+0.6}{-0.6} \\
  Jet energy scale & \asymerr{+0.6}{-0.9} & \asymerr{+1.0}{-0.5} & \asymerr{+0.1}{-1.3} & \asymerr{+1.7}{-0.7} \\
  Flavour tagging & \asymerr{+0.0}{-0.0} & \asymerr{+0.0}{-0.0} & \asymerr{+0.0}{-0.0} & \asymerr{+0.1}{-0.1} \\
  \MET modelling & \asymerr{+0.3}{-0.0} & \asymerr{+0.3}{-0.6} & \asymerr{+0.1}{-0.6} & \asymerr{+0.9}{-0.0} \\
  PDF & \asymerr{+0.9}{-0.9} & \asymerr{+3.5}{-3.5} & \asymerr{+1.1}{-1.2} & \asymerr{+5.2}{-5.2} \\
  \tq (\tbarq) NLO matching & \asymerr{+5.0}{-5.0} & \asymerr{+4.5}{-4.5} & \asymerr{+5.7}{-5.7} & \asymerr{+8.4}{-8.4} \\
  \tq (\tbarq) parton shower & \asymerr{+0.5}{-0.5} & \asymerr{+3.0}{-3.0} & \asymerr{+1.6}{-1.6} & \asymerr{+0.8}{-0.8} \\
  \tq (\tbarq) scale variations & \asymerr{+0.0}{-2.5} & \asymerr{+0.2}{-0.5} & \asymerr{+3.3}{-1.0} & \asymerr{+3.2}{-2.5} \\
  \ttbar NLO matching & \asymerr{+0.7}{-0.7} & \asymerr{+1.0}{-1.0} & \asymerr{+1.8}{-1.8} & \asymerr{+0.9}{-0.9} \\
  \ttbar parton shower & \asymerr{+1.4}{-1.4} & \asymerr{+3.2}{-3.2} & \asymerr{+1.0}{-1.0} & \asymerr{+0.8}{-0.8} \\
  \ttbar scale variations & \asymerr{+0.0}{-0.9} & \asymerr{+0.0}{-0.2} & \asymerr{+0.0}{-1.9} & \asymerr{+3.7}{-0.0} \\
\midrule
  Total systematic & \asymerr{+5.8}{-6.4} & \asymerr{+7.4}{-7.4} & \asymerr{+8.1}{-7.9} & \asymerr{+13}{-12} \\
  Total (stat.\ + syst.) & \asymerr{+10}{-10} & \asymerr{+11}{-11} & \asymerr{+11}{-10} & \asymerr{+16}{-16} \\


==> systopY_minus_summary.tex <==
Source of uncertainty      & \multicolumn{2}{c}{Bin 1}      & \multicolumn{2}{c}{Bin 2}      & \multicolumn{2}{c}{Bin 3}      & \multicolumn{2}{c}{Bin 4}        \\
& \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}        \\
\midrule
\endhead
  Data statistics & \symerr{7.9} & \symerr{8.7} & \symerr{7.2} & \symerr{11} \\
  Monte Carlo statistics & \symerr{0.9} & \symerr{0.8} & \symerr{0.7} & \symerr{1.0} \\
\midrule
  Unfolding & \asymerr{+0.1}{-0.1} & \asymerr{+0.4}{-0.4} & \asymerr{+2.7}{-2.7} & \asymerr{+5.1}{-5.1} \\
  Background normalisation & \asymerr{+4.1}{-4.1} & \asymerr{+5.2}{-5.2} & \asymerr{+5.3}{-5.3} & \asymerr{+8.7}{-8.7} \\
  Background modelling & \asymerr{+0.8}{-0.8} & \asymerr{+0.4}{-0.4} & \asymerr{+2.0}{-2.0} & \asymerr{+3.5}{-3.5} \\
  Lepton reconstruction & \asymerr{+1.9}{-1.9} & \asymerr{+1.9}{-1.9} & \asymerr{+1.9}{-2.0} & \asymerr{+1.9}{-1.9} \\
  Jet reconstruction & \asymerr{+0.8}{-0.8} & \asymerr{+1.1}{-1.1} & \asymerr{+1.8}{-1.8} & \asymerr{+0.5}{-0.5} \\
  Jet energy scale & \asymerr{+2.1}{-2.0} & \asymerr{+2.6}{-1.4} & \asymerr{+1.8}{-2.7} & \asymerr{+4.1}{-2.7} \\
  Flavour tagging & \asymerr{+1.2}{-1.2} & \asymerr{+1.2}{-1.2} & \asymerr{+1.1}{-1.1} & \asymerr{+1.2}{-1.2} \\
  \MET modelling & \asymerr{+0.5}{-0.1} & \asymerr{+0.6}{-0.5} & \asymerr{+0.2}{-0.7} & \asymerr{+0.9}{-0.0} \\
  $b/\bbar$ efficiency & \symerr{0.9} & \symerr{0.9} & \symerr{0.9} & \symerr{0.9} \\
  PDF & \asymerr{+1.2}{-1.2} & \asymerr{+3.0}{-3.0} & \asymerr{+0.6}{-0.7} & \asymerr{+5.8}{-5.8} \\
  \tq (\tbarq) NLO matching & \asymerr{+5.8}{-5.8} & \asymerr{+3.7}{-3.7} & \asymerr{+4.8}{-4.8} & \asymerr{+9.2}{-9.2} \\
  \tq (\tbarq) parton shower & \asymerr{+0.6}{-0.6} & \asymerr{+2.9}{-2.9} & \asymerr{+1.6}{-1.6} & \asymerr{+0.9}{-0.9} \\
  \tq (\tbarq) scale variations & \asymerr{+0.0}{-2.6} & \asymerr{+0.1}{-0.0} & \asymerr{+3.2}{-0.5} & \asymerr{+3.6}{-2.6} \\
  \ttbar NLO matching & \asymerr{+0.6}{-0.6} & \asymerr{+0.9}{-0.9} & \asymerr{+1.9}{-1.9} & \asymerr{+0.8}{-0.8} \\
  \ttbar parton shower & \asymerr{+1.5}{-1.5} & \asymerr{+3.1}{-3.1} & \asymerr{+1.2}{-1.2} & \asymerr{+0.9}{-0.9} \\
  \ttbar scale variations & \asymerr{+0.0}{-0.8} & \asymerr{+0.3}{-0.0} & \asymerr{+0.0}{-1.5} & \asymerr{+4.1}{-0.0} \\
  Luminosity & \symerr{1.9} & \symerr{1.9} & \symerr{1.9} & \symerr{1.9} \\
\midrule
  Total systematic & \asymerr{+8.4}{-8.8} & \asymerr{+9.3}{-9.1} & \asymerr{+10}{-10} & \asymerr{+17}{-16} \\
  Total (stat.\ + syst.) & \asymerr{+12}{-12} & \asymerr{+13}{-13} & \asymerr{+12}{-12} & \asymerr{+20}{-20} \\


==> systopY_plus_XS_summary.tex <==
Source of uncertainty      & \multicolumn{2}{c}{Bin 1}      & \multicolumn{2}{c}{Bin 2}      & \multicolumn{2}{c}{Bin 3}      & \multicolumn{2}{c}{Bin 4}        \\
& \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}        \\
\midrule
\endhead
  Data statistics & \symerr{5.5} & \symerr{5.5} & \symerr{4.8} & \symerr{4.8} \\
  Monte Carlo statistics & \symerr{0.7} & \symerr{0.6} & \symerr{0.6} & \symerr{0.7} \\
\midrule
  Unfolding & \asymerr{+2.7}{-2.7} & \asymerr{+1.2}{-1.2} & \asymerr{+0.2}{-0.2} & \asymerr{+3.4}{-3.4} \\
  Background normalisation & \asymerr{+0.9}{-0.9} & \asymerr{+0.5}{-0.5} & \asymerr{+0.3}{-0.3} & \asymerr{+0.8}{-0.8} \\
  Background modelling & \asymerr{+0.0}{-0.0} & \asymerr{+0.0}{-0.0} & \asymerr{+0.0}{-0.0} & \asymerr{+0.0}{-0.0} \\
  Lepton reconstruction & \asymerr{+0.3}{-0.2} & \asymerr{+0.3}{-0.3} & \asymerr{+0.2}{-0.2} & \asymerr{+0.5}{-0.4} \\
  Jet reconstruction & \asymerr{+2.5}{-2.5} & \asymerr{+2.3}{-2.3} & \asymerr{+1.1}{-1.1} & \asymerr{+0.9}{-0.9} \\
  Jet energy scale & \asymerr{+0.8}{-1.6} & \asymerr{+1.2}{-0.8} & \asymerr{+0.8}{-0.4} & \asymerr{+1.2}{-1.1} \\
  Flavour tagging & \asymerr{+0.1}{-0.1} & \asymerr{+0.0}{-0.0} & \asymerr{+0.0}{-0.0} & \asymerr{+0.1}{-0.1} \\
  \MET modelling & \asymerr{+0.0}{-0.6} & \asymerr{+0.5}{-0.0} & \asymerr{+0.0}{-0.4} & \asymerr{+0.5}{-0.0} \\
  PDF & \asymerr{+2.2}{-2.2} & \asymerr{+0.6}{-0.6} & \asymerr{+2.2}{-2.2} & \asymerr{+1.5}{-1.5} \\
  \tq (\tbarq) NLO matching & \asymerr{+0.4}{-0.4} & \asymerr{+3.5}{-3.5} & \asymerr{+4.0}{-4.0} & \asymerr{+1.7}{-1.7} \\
  \tq (\tbarq) parton shower & \asymerr{+3.7}{-3.7} & \asymerr{+0.3}{-0.3} & \asymerr{+1.6}{-1.6} & \asymerr{+0.7}{-0.7} \\
  \tq (\tbarq) scale variations & \asymerr{+4.5}{-0.0} & \asymerr{+0.2}{-2.1} & \asymerr{+0.0}{-1.4} & \asymerr{+0.0}{-1.3} \\
  \ttbar NLO matching & \asymerr{+0.3}{-0.3} & \asymerr{+0.9}{-0.9} & \asymerr{+0.8}{-0.8} & \asymerr{+1.4}{-1.4} \\
  \ttbar parton shower & \asymerr{+0.4}{-0.4} & \asymerr{+1.5}{-1.5} & \asymerr{+0.8}{-0.8} & \asymerr{+0.1}{-0.1} \\
  \ttbar scale variations & \asymerr{+0.0}{-0.3} & \asymerr{+0.0}{-0.7} & \asymerr{+0.6}{-0.0} & \asymerr{+0.4}{-0.5} \\
\midrule
  Total systematic & \asymerr{+7.4}{-6.1} & \asymerr{+5.0}{-5.4} & \asymerr{+5.2}{-5.4} & \asymerr{+4.8}{-4.9} \\
  Total (stat.\ + syst.) & \asymerr{+9.2}{-8.2} & \asymerr{+7.4}{-7.7} & \asymerr{+7.1}{-7.2} & \asymerr{+6.8}{-6.9} \\


==> systopY_plus_summary.tex <==
Source of uncertainty      & \multicolumn{2}{c}{Bin 1}      & \multicolumn{2}{c}{Bin 2}      & \multicolumn{2}{c}{Bin 3}      & \multicolumn{2}{c}{Bin 4}        \\
& \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}         & \multicolumn{2}{c}{[\%]}        \\
\midrule
\endhead
  Data statistics & \symerr{5.6} & \symerr{5.6} & \symerr{5.0} & \symerr{5.7} \\
  Monte Carlo statistics & \symerr{0.8} & \symerr{0.7} & \symerr{0.6} & \symerr{0.8} \\
\midrule
  Unfolding & \asymerr{+2.3}{-2.3} & \asymerr{+0.8}{-0.8} & \asymerr{+0.2}{-0.2} & \asymerr{+3.8}{-3.8} \\
  Background normalisation & \asymerr{+2.5}{-2.5} & \asymerr{+3.0}{-3.0} & \asymerr{+3.7}{-3.7} & \asymerr{+4.2}{-4.2} \\
  Background modelling & \asymerr{+0.0}{-0.0} & \asymerr{+0.0}{-0.0} & \asymerr{+0.0}{-0.0} & \asymerr{+0.0}{-0.0} \\
  Lepton reconstruction & \asymerr{+1.9}{-1.9} & \asymerr{+1.9}{-1.9} & \asymerr{+1.9}{-1.9} & \asymerr{+2.0}{-1.9} \\
  Jet reconstruction & \asymerr{+1.1}{-1.1} & \asymerr{+3.6}{-3.6} & \asymerr{+0.2}{-0.2} & \asymerr{+2.2}{-2.2} \\
  Jet energy scale & \asymerr{+1.0}{-1.7} & \asymerr{+2.2}{-2.1} & \asymerr{+2.1}{-1.3} & \asymerr{+2.8}{-2.9} \\
  Flavour tagging & \asymerr{+1.2}{-1.2} & \asymerr{+1.2}{-1.2} & \asymerr{+1.2}{-1.2} & \asymerr{+1.2}{-1.2} \\
  \MET modelling & \asymerr{+0.0}{-0.5} & \asymerr{+0.5}{-0.0} & \asymerr{+0.1}{-0.4} & \asymerr{+0.5}{-0.0} \\
  $b/\bbar$ efficiency & \symerr{0.9} & \symerr{0.9} & \symerr{0.9} & \symerr{0.9} \\
  PDF & \asymerr{+1.9}{-1.9} & \asymerr{+0.5}{-0.6} & \asymerr{+2.4}{-2.4} & \asymerr{+1.4}{-1.4} \\
  \tq (\tbarq) NLO matching & \asymerr{+0.6}{-0.6} & \asymerr{+3.2}{-3.2} & \asymerr{+4.3}{-4.3} & \asymerr{+1.4}{-1.4} \\
  \tq (\tbarq) parton shower & \asymerr{+3.4}{-3.4} & \asymerr{+0.5}{-0.5} & \asymerr{+1.9}{-1.9} & \asymerr{+0.9}{-0.9} \\
  \tq (\tbarq) scale variations & \asymerr{+4.0}{-0.0} & \asymerr{+0.0}{-2.5} & \asymerr{+0.0}{-1.8} & \asymerr{+0.0}{-1.7} \\
  \ttbar NLO matching & \asymerr{+0.5}{-0.5} & \asymerr{+0.7}{-0.7} & \asymerr{+0.6}{-0.6} & \asymerr{+1.6}{-1.6} \\
  \ttbar parton shower & \asymerr{+0.5}{-0.5} & \asymerr{+1.4}{-1.4} & \asymerr{+0.9}{-0.9} & \asymerr{+0.2}{-0.2} \\
  \ttbar scale variations & \asymerr{+0.0}{-0.3} & \asymerr{+0.0}{-0.6} & \asymerr{+0.5}{-0.0} & \asymerr{+0.5}{-0.6} \\
  Luminosity & \symerr{1.9} & \symerr{1.9} & \symerr{1.9} & \symerr{1.9} \\
\midrule
  Total systematic & \asymerr{+7.5}{-6.5} & \asymerr{+7.1}{-7.5} & \asymerr{+7.6}{-7.6} & \asymerr{+7.9}{-8.1} \\
  Total (stat.\ + syst.) & \asymerr{+9.3}{-8.6} & \asymerr{+9.1}{-9.4} & \asymerr{+9.1}{-9.1} & \asymerr{+10}{-10} \\


==> xsect_diff_syst.tex <==
%-------------------------------------------------------------------------------
\section{Uncertainties on the differential cross-sections}
\label{sec:xsect_diff_sys}
%-------------------------------------------------------------------------------

This section contains a series of tables with the statistical 
and a breakdown of the systematic uncertainties
for the differential cross-section measurements.
It uses the same categories as in \Tab{\ref{tab:xs-uncertainty}}.
A more detailed breakdown will be provided in HepData format.

%-------------------------------------------------------------------------------
% Systematics for top pT at particle level
\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{7}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{14}{c}{Uncertainties on $\dif\sigma(\tq) / \dif\pTthat$ at particle level}\\
    \input{tables/particle/systopPt_plus_summary}
    \bottomrule
    \caption{Uncertainties for the absolute differential \tq cross-section as a function of \pTthat at particle level
      per bin ($[0,35,50,75,100,150,200,300]\;\si{\GeV}$) in percent
      of $\dif\sigma(\tq) / \dif\pTthat$.}
    \label{tab:topPT:ptcl}
  \end{longtable}
\end{sidewaystable}
%\clearpage

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{7}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{14}{c}{Uncertainties on $(1/\sigma) \dif\sigma(\tq) / \dif\pTthat$ at particle level}\\
    \input{tables/particle/systopPt_plus_XS_summary}
    \bottomrule
    \caption{Uncertainties for the normalised differential \tq cross-section as a function of \pTthat at particle level
      per bin ($[0,35,50,75,100,150,200,300]\;\si{\GeV}$) in percent
      of $(1/\sigma) \dif\sigma(\tq) / \dif\pTthat$.}
    \label{tab:topPT:ptcl_norm}
  \end{longtable}
\end{sidewaystable}
%\clearpage

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{6}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{12}{c}{Uncertainties on $\dif\sigma(\tbarq) / \dif\pTthat$ at particle level}\\
    \input{tables/particle/systopPt_minus_summary}
    \bottomrule
    \caption{Uncertainties for the absolute differential \tbarq cross-section as a function of \pTthat at particle level
      per bin ($[0,35,50,75,100,150,300]\;\si{\GeV}$) in percent
      of $\dif\sigma(\tbarq) / \dif\pTthat$.}
    \label{tab:antitopPT:ptcl}
  \end{longtable}
\end{sidewaystable}
%\clearpage

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{6}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{12}{c}{Uncertainties on $(1/\sigma) \dif\sigma(\tbarq) / \dif\pTthat$ at particle level}\\
    \input{tables/particle/systopPt_minus_XS_summary}
    \bottomrule
    \caption{Uncertainties for the normalised differential \tbarq cross-section as a function of \pTthat at particle level
      per bin ($[0,35,50,75,100,150,300]\;\si{\GeV}$) in percent
      of $(1/\sigma) \dif\sigma(\tbarq) / \dif\pTthat$.}
    \label{tab:antitopPT:ptcl_norm}
  \end{longtable}
\end{sidewaystable}
%\clearpage


%-------------------------------------------------------------------------------
% Systematics for top rapidity at particle level
\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}{l
      *{7}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{14}{c}{Uncertainties on $\dif\sigma(\tq) / \dif\absythat$ at particle level}\\
    \input{tables/particle/systopY_plus_summary}
    \bottomrule
    \caption{Uncertainties for the absolute differential \tq cross-section as a function of \absythat at particle level
      per bin ($[0,0.15,0.3,0.45,0.7,1.0,1.3,2.2]$) in percent
      of $\dif\sigma(\tq) / \dif\absythat$.}
    \label{tab:topY:ptcl}
  \end{longtable}
\end{sidewaystable}

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}{l
      *{7}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{14}{c}{Uncertainties on $(1/\sigma) \dif\sigma(\tq) / \dif\absythat$ at particle level}\\
    \input{tables/particle/systopY_plus_XS_summary}
    \bottomrule
    \caption{Uncertainties for the normalised differential \tq cross-section as a function of \absythat at particle level
      per bin ($[0,0.15,0.3,0.45,0.7,1.0,1.3,2.2]$) in percent
      of $(1/\sigma) \dif\sigma(\tq) / \dif\absythat$.}
    \label{tab:topY:ptcl_norm}
  \end{longtable}
\end{sidewaystable}

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{7}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{14}{c}{Uncertainties on $\dif\sigma(\tq) / \dif\absythat$ at particle level}\\
    \input{tables/particle/systopY_minus_summary}
    \bottomrule
    \caption{Uncertainties for the absolute differential \tbarq cross-section as a function of \absythat at particle level
      per bin ($[0,0.15,0.3,0.45,0.7,1.0,1.3,2.2]$) in percent
      of $\dif\sigma(\tbarq) / \dif\absythat$.}
    \label{tab:antitopY:ptcl}
  \end{longtable}
\end{sidewaystable}

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{7}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{14}{c}{Uncertainties on $(1/\sigma) \dif\sigma(\tbarq) / \dif\absythat$ at particle level}\\
    \input{tables/particle/systopY_minus_XS_summary}
    \bottomrule
    \caption{Uncertainties for the absolute differential \tbarq cross-section as a function of \absythat at particle level
      per bin ($[0,0.15,0.3,0.45,0.7,1.0,1.3,2.2]$) in percent
      of $(1/\sigma) \dif\sigma(\tbarq) / \dif\absythat$.}
    \label{tab:antitopY:ptcl_norm}
  \end{longtable}
\end{sidewaystable}


%-------------------------------------------------------------------------------
% Systematics for light-parton-jet pT at particle level
\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{6}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{12}{c}{Uncertainties on $\dif\sigma(\tq) / \dif\pTjhat$ at particle level}\\
    \input{tables/particle/syslightPt_plus_summary}
    \bottomrule
    \caption{Uncertainties for the absolute differential \tq cross-section as a function of \pTjhat at particle level
      per bin ($[30,45,60,75,100,150,300]\;\si{\GeV}$) in percent
      of $\dif\sigma(\tq) / \pTjhat$.}
    \label{tab:plulightpT:ptcl}
  \end{longtable}
\end{sidewaystable}

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{6}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{12}{c}{Uncertainties on $(1/\sigma) \dif\sigma(\tq) / \dif\pTjhat$ at particle level}\\
    \input{tables/particle/syslightPt_plus_XS_summary}
    \bottomrule
    \caption{Uncertainties for the normalised differential \tq cross-section as a function of \pTjhat at particle level
      per bin ($[30,45,60,75,100,150,300]\;\si{\GeV}$) in percent
      of $(1/\sigma) \dif\sigma(\tq) / \pTjhat$.}
    \label{tab:plulightpT:ptcl_norm}
  \end{longtable}
\end{sidewaystable}

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{6}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{12}{c}{Uncertainties on $\dif\sigma(\tbarq) / \dif\pTjhat$ at particle level}\\
    \input{tables/particle/syslightPt_minus_summary}
    \bottomrule
    \caption{Uncertainties for the absolute differential \tbarq cross-section as a function of \pTjhat at particle level
      per bin ($[30,45,60,75,100,150,300]\;\si{\GeV}$) in percent
      of $\dif\sigma(\tbarq) / \dif\pTjhat$.}
    \label{tab:minlightpT:ptcl}
  \end{longtable}
\end{sidewaystable}

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{6}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{12}{c}{Uncertainties on $\dif\sigma(\tbarq) / \dif\pTjhat$ at particle level}\\
    \input{tables/particle/syslightPt_minus_XS_summary}
    \bottomrule
    \caption{Uncertainties for the normalised differential \tbarq cross-section as a function of \pTjhat at particle level
      per bin ($[30,45,60,75,100,150,300]\;\si{\GeV}$) in percent
      of $(1/\sigma) \dif\sigma(\tbarq) / \dif\pTjhat$.}
    \label{tab:minlightpT:ptcl_norm}
  \end{longtable}
\end{sidewaystable}


%-------------------------------------------------------------------------------
% Systematics for light-parton-jet y at particle level
\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{7}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{14}{c}{Uncertainties on $\dif\sigma(\tq) / \dif\absyjhat$ at particle level}\\
    \input{tables/particle/syslighty_plus_summary}
    \bottomrule
    \caption{Uncertainties for the absolute differential \tq cross-section as a function of \absyjhat at particle level
      per bin ($[30,45,60,75,100,150,300]\;\si{\GeV}$) in percent
      of $\dif\sigma(\tq) / \absyjhat$.}
    \label{tab:plulighty:ptcl}
  \end{longtable}
\end{sidewaystable}

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{7}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{14}{c}{Uncertainties on $(1/\sigma) \dif\sigma(\tq) / \dif\absyjhat$ at particle level}\\
    \input{tables/particle/syslighty_plus_XS_summary}
    \bottomrule
    \caption{Uncertainties for the normalised differential \tq cross-section as a function of \absyjhat at particle level
      per bin ($[30,45,60,75,100,150,300]\;\si{\GeV}$) in percent
      of $(1/\sigma) \dif\sigma(\tq) / \absyjhat$.}
    \label{tab:plulighty:ptcl_norm}
  \end{longtable}
\end{sidewaystable}

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{7}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{14}{c}{Uncertainties on $\dif\sigma(\tbarq) / \dif\absyjhat$ at particle level}\\
    \input{tables/particle/syslighty_minus_summary}
    \bottomrule
    \caption{Uncertainties for the absolute differential \tbarq cross-section as a function of \absyjhat at particle level
      per bin ($[30,45,60,75,100,150,300]\;\si{\GeV}$) in percent
      of $\dif\sigma(\tbarq) / \dif\absyjhat$.}
    \label{tab:minlighty:ptcl}
  \end{longtable}
\end{sidewaystable}

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{7}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{14}{c}{Uncertainties on $(1/\sigma) \dif\sigma(\tbarq) / \dif\absyjhat$ at particle level}\\
    \input{tables/particle/syslighty_minus_XS_summary}
    \bottomrule
    \caption{Uncertainties for the normalised differential \tbarq cross-section as a function of \absyjhat at particle level
      per bin ($[30,45,60,75,100,150,300]\;\si{\GeV}$) in percent
      of $(1/\sigma) \dif\sigma(\tbarq) / \dif\absyjhat$.}
    \label{tab:minlighty:ptcl_norm}
  \end{longtable}
\end{sidewaystable}


%-------------------------------------------------------------------------------
% Systematics for top pT at parton level
\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{5}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{10}{c}{Uncertainties on $\dif\sigma(\tq) / \dif\pTthat$ at parton level}\\
    \input{tables/parton/systopPt_plus_summary}
    \bottomrule
    \caption{Uncertainties for the absolute differential \tq cross-section as a function of \pTthat at parton level
      per bin ($[0,35,50,75,100,150,200,300]\;\si{\GeV}$) in percent
      of $\dif\sigma(\tq) / \dif\pTthat$.}
    \label{tab:topPT:prtn}
  \end{longtable}
\end{sidewaystable}
%\clearpage

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{5}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{10}{c}{Uncertainties on $(1/\sigma) \dif\sigma(\tq) / \dif\pTthat$ at parton level}\\
    \input{tables/parton/systopPt_plus_XS_summary}
    \bottomrule
    \caption{Uncertainties for the normalised differential \tq cross-section as a function of \pTthat at parton level
      per bin ($[0,35,50,75,100,150,200,300]\;\si{\GeV}$) in percent
      of $(1/\sigma) \dif\sigma(\tq) / \dif\pTthat$.}
    \label{tab:topPT:prtn_norm}
  \end{longtable}
\end{sidewaystable}
% WW: We need this clearpage, otherwise the remaining floats are not plotted by
% LateX since there are too many unprocessed floats.
\clearpage

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{4}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{8}{c}{Uncertainties on $\dif\sigma(\tbarq) / \dif\pTthat$ at parton level}\\
    \input{tables/parton/systopPt_minus_summary}
    \bottomrule
    \caption{Uncertainties for the absolute differential \tbarq cross-section as a function of \pTthat at parton level
      per bin ($[0,35,50,75,100,150,300]\;\si{\GeV}$) in percent
      of $\dif\sigma(\tbarq) / \dif\pTthat$.}
    \label{tab:antitopPT:prtn}
  \end{longtable}
\end{sidewaystable}
%\clearpage

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{4}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{8}{c}{Uncertainties on $(1/\sigma) \dif\sigma(\tbarq) / \dif\pTthat$ at parton level}\\
    \input{tables/parton/systopPt_minus_XS_summary}
    \bottomrule
    \caption{Uncertainties for the normalised differential \tbarq cross-section as a function of \pTthat at parton level
      per bin ($[0,35,50,75,100,150,300]\;\si{\GeV}$) in percent
      of $(1/\sigma) \dif\sigma(\tbarq) / \dif\pTthat$.}
    \label{tab:antitopPT:prtn_norm}
  \end{longtable}
\end{sidewaystable}
%\clearpage


%-------------------------------------------------------------------------------
% Systematics for top rapidity at parton level
\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}{l
      *{4}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{8}{c}{Uncertainties on $\dif\sigma(\tq) / \dif\absythat$ at parton level}\\
    \input{tables/parton/systopY_plus_summary}
    \bottomrule
    \caption{Uncertainties for the absolute differential \tq cross-section as a function of \absythat at parton level
      per bin ($[0,0.15,0.3,0.45,0.7,1.0,1.3,2.2]$) in percent
      of $\dif\sigma(\tq) / \dif\absythat$.}
    \label{tab:topY:prtn}
  \end{longtable}
\end{sidewaystable}

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}{l
      *{4}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    & \multicolumn{8}{c}{Uncertainties on $(1/\sigma) \dif\sigma(\tq) / \dif\absythat$ at parton level}\\
    \input{tables/parton/systopY_plus_XS_summary}
    \bottomrule
    \caption{Uncertainties for the normalised differential \tq cross-section as a function of \absythat at parton level
      per bin ($[0,0.15,0.3,0.45,0.7,1.0,1.3,2.2]$) in percent
      of $(1/\sigma) \dif\sigma(\tq) / \dif\absythat$.}
    \label{tab:topY:prtn_norm}
  \end{longtable}
\end{sidewaystable}

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{4}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    %& \multicolumn{8}{c}{Uncertainties on $\dif\sigma(\tq) / \dif\absythat$ at parton level}\\
    \input{tables/parton/systopY_minus_summary}
    \bottomrule
    \caption{Uncertainties for the absolute differential \tbarq cross-section as a function of \absythat at parton level
      per bin ($[0,0.15,0.3,0.45,0.7,1.0,1.3,2.2]$) in percent
      of $\dif\sigma(\tbarq) / \dif\absythat$.}
    \label{tab:antitopY:prtn}
  \end{longtable}
\end{sidewaystable}

\begin{sidewaystable}
  \sisetup{retain-explicit-plus}
  \begin{longtable}[c]{l
      *{4}{S[table-format=-2.1, parse-numbers=false]@{\,/\,}S[table-format=-2.1, parse-numbers=false]}
    }
    \toprule
    %& \multicolumn{8}{c}{Uncertainties on $(1/\sigma) \dif\sigma(\tq) / \dif\absythat$ at parton level}\\
    \input{tables/parton/systopY_minus_XS_summary}
    \bottomrule
    \caption{Uncertainties for the normalised differential \tbarq cross-section as a function of \absythat at parton level
      per bin ($[0,0.15,0.3,0.45,0.7,1.0,1.3,2.2]$) in percent
      of $(1/\sigma) \dif\sigma(\tbarq) / \dif\absythat$.}
    \label{tab:antitopY:prtn_norm}
  \end{longtable}
\end{sidewaystable}

